The Farthest Point Map on the Regular Octahedron

On any compact space one can consider the map which sends a point to the set of points farthest from this point. In nice cases, there is just a single point farthest from a given point and so by restricting the domain slightly one can form a dynamical system on the space based on this map. We give a complete characterization of this map, including explicit formulas, when the metric space is the regular octahedron equipped with its intrinsic flat cone metric.

==> 5final.tex <==
\section{The Vertex Competition}
\label{final0}

